OpenOmni: A Collaborative Open Source Tool for Building Future-Ready Multimodal Conversational Agents

Multimodal conversational agents are highly desirable because they offer natural and human-like interaction. However, there is a lack of comprehensive end-to-end solutions to support collaborative development and benchmarking. While proprietary systems like GPT-4o and Gemini demonstrating impressive integration of audio, video, and text with response times of 200-250ms, challenges remain in balancing latency, accuracy, cost, and data privacy. To better understand and quantify these issues, we developed OpenOmni, an open-source, end-to-end pipeline benchmarking tool that integrates advanced technologies such as Speech-to-Text, Emotion Detection, Retrieval Augmented Generation, Large Language Models, along with the ability to integrate customized models. OpenOmni supports local and cloud deployment, ensuring data privacy and supporting latency and accuracy benchmarking. This flexible framework allows researchers to customize the pipeline, focusing on real bottlenecks and facilitating rapid proof-of-concept development. OpenOmni can significantly enhance applications like indoor assistance for visually impaired individuals, advancing human-computer interaction. Our demonstration video is available https://www.youtube.com/watch?v=zaSiT3clWqY, demo is available via https://openomni.ai4wa.com, code is available via https://github.com/AI4WA/OpenOmniFramework.

==> libs/preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This file contains the packages that can be used in the beamer. %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Package to fonts family
\usepackage[T1]{fontenc}
% Package to accentuation
\usepackage[utf8]{inputenc}
% Package to Portuguese language
%\usepackage[brazil]{babel}
% Package to Figures
\usepackage{graphicx}
% Package for clipping
\usepackage{adjustbox}
%\usepackage{wrapfigure}
% Package for citation
\usepackage{natbib}
% Package to the colors
\usepackage{color}
% Package to the colors
\usepackage{xcolor}
% Packages to math symbols and expressions
\usepackage{amsfonts, amssymb, amsmath}
% Package to multiple lines and columns in table
\usepackage{multirow, array} 
% Package to create pseudo-code
% For more detail of this package: http://linorg.usp.br/CTAN/macros/latex/contrib/algorithm2e/doc/algorithm2e.pdf
\usepackage{algorithm2e}
% Package to insert code
\usepackage{listings} 
\usepackage{keyval}
% Package to justify text
\usepackage[document]{ragged2e}
% Package to manage the bibliography
%\usepackage[backend=biber, style=numeric, sorting=none]{biblatex}
% Package to facilities quotations
\usepackage{csquotes}
% Package to use multicols
\usepackage{multicol}
% Package to use tikz and its libraries
\usepackage{tikz}
\usetikzlibrary{er,positioning}
\usetikzlibrary{graphs,graphdrawing,quotes}
\usegdlibrary{force, layered, trees}
% Package for left aligned nested matrices
\usepackage{mathtools}
% Package for alternating color in table rows
%\usepackage{xcolor}
\definecolor{lightgray}{gray}{0.9}
\let\oldtabular\tabular
\let\endoldtabular\endtabular
\renewenvironment{tabular}{\rowcolors{2}{white}{lightgray}\oldtabular}{\endoldtabular}
\usepackage{listings}
\usepackage{array}

% Define citation alias
\defcitealias{NLP_Embeddings}{Embeddings~in~NLP}
\defcitealias{Neural_MT}{Neural~Machine~Translation}
\defcitealias{Statistical_MT}{Statistical~Machine~Translation}
\defcitealias{NLP_Pytorch}{NLP~with~PyTorch}
\defcitealias{NLP_Spacy}{NLP~with~Python~and~spaCy}
\defcitealias{DL_Pytorch}{Deep~Learning~with~Pytorch~Step~by~Step}


% Create a title page for each section
\AtBeginSection[]{
  \begin{frame}
  \vfill
  \centering
  \begin{beamercolorbox}[sep=8pt,center,shadow=true,rounded=true]{title}
    \usebeamerfont{title}\insertsectionhead\par%
  \end{beamercolorbox}
  \vfill
  \end{frame}
}
% short hyphen
\mathchardef\mhyphen="2D
\newcommand\tfidf{\mathit{tf\mhyphen idf}}

% https://pythonawesome.com/deep-learning-with-pytorch-step-by-step-a-beginners-guide/

\usepackage{libs/kbordermatrix}

%% argmin and argmax
\newcommand{\argmin}{\arg\!\min}
\newcommand{\argmax}{\arg\!\max}

\usepackage{emoji}
